DSAG: A mixed synchronous-asynchronous iterative method for straggler-resilient learning

We consider straggler-resilient learning. In many previous works, e.g., in the coded computing literature, straggling is modeled as random delays that are independent and identically distributed between workers. However, in many practical scenarios, a given worker may straggle over an extended period of time. We propose a latency model that captures this behavior and is substantiated by traces collected on Microsoft Azure, Amazon Web Services (AWS), and a small local cluster. Building on this model, we propose DSAG, a mixed synchronous-asynchronous iterative optimization method, based on the stochastic average gradient (SAG) method, that combines timely and stale results. We also propose a dynamic load-balancing strategy to further reduce the impact of straggling workers. We evaluate DSAG for principal component analysis, cast as a finite-sum optimization problem, of a large genomics dataset, and for logistic regression on a cluster composed of 100 workers on AWS, and find that DSAG is up to about 50% faster than SAG, and more than twice as fast as coded computing methods, for the particular scenario that we consider.

==> figures/orderstats/grid.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{HTML}{75b9be}
\definecolor{color1}{HTML}{ee7674}
\definecolor{color2}{HTML}{832161}
\definecolor{color3}{HTML}{eab464}
\definecolor{color4}{HTML}{335145}

% Azure job 39 (2.84e6)
\begin{axis}[
name=plot1,
legend cell align={left},
legend style={font=\scriptsize, fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.02,0.98)}, anchor=north west, draw=white!80!black},
tick pos=left,
tick label style={font=\scriptsize},
grid style={gray,opacity=0.5,dotted},
xtick distance=20,
xmajorgrids,
height=\figureheight,
width=0.68\figurewidth,
xmin=0, xmax=80,
ylabel={Latency [s]},
ymajorgrids,
ymin=4e-3, ymax=9e-3,
ytick distance=1e-3,
]

\addplot [semithick, color0]
table {./figures/orderstats/data/azure/orderstats_39.csv};
\addlegendentry{Empirical}

\addplot [semithick, only marks, color2, mark=square*, mark size=1, mark options={fill=white,solid}] 
table {./figures/orderstats/data/azure/orderstats_gamma_gamma_39.csv};
\addlegendentry{Predicted}

\addplot [semithick, color3, mark=*, only marks, mark size=1, mark options={fill=white,solid}] 
table {./figures/orderstats/data/azure/orderstats_gamma_gamma_copula_39.csv};
\addlegendentry{Predicted (corr.)}

\addplot [semithick, only marks, color1, mark=triangle*, mark size=1, mark options={fill=white,solid}] 
table {./figures/orderstats/data/azure/orderstats_global_gamma_39.csv};
\addlegendentry{Predicted (i.i.d.)}

\end{axis}%
%
% Azure job 35 (1.13e7)
\begin{axis}[
name=plot2,
at=(plot1.below south west), anchor=above north west,
legend cell align={left},
legend style={font=\scriptsize, fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.02,0.98)}, anchor=north west, draw=white!80!black},
tick label style={font=\scriptsize},
tick pos=left,
grid style={gray,opacity=0.5,dotted},
xtick distance=20,
xmajorgrids,
height=\figureheight,
width=0.68\figurewidth,
xmin=0, xmax=80,
ylabel={Latency [s]},
ymajorgrids,
ymin=1.4e-2, ymax=2.2e-2,
% ytick distance=1e-3,
]

\addplot [semithick, color0]
table {./figures/orderstats/data/azure/orderstats_35.csv};

\addplot [semithick, dashed, only marks, color2, mark=square*, mark size=1, mark options={fill=white,solid}] 
table {./figures/orderstats/data/azure/orderstats_gamma_gamma_35.csv};

\addplot [semithick, dashed, color3, mark=pentagon*, mark size=1, mark options={fill=white,solid}] 
table {./figures/orderstats/data/azure/orderstats_gamma_gamma_copula_35.csv};

\addplot [semithick, dashed, only marks, color1, mark=triangle*, mark size=1, mark options={fill=white,solid}] 
table {./figures/orderstats/data/azure/orderstats_global_gamma_35.csv};

\end{axis}%
%
% Azure job 2 (4.54e8)
\begin{axis}[
name=plot3,
at=(plot2.below south west), anchor=above north west,
legend cell align={left},
legend style={font=\scriptsize, fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.02,0.98)}, anchor=north west, draw=white!80!black},
tick pos=left,
tick label style={font=\scriptsize},
grid style={gray,opacity=0.5,dotted},
xlabel style={align=center}, xlabel={$w$},
xtick distance=20,
xmajorgrids,
height=\figureheight,
width=0.68\figurewidth,
xmin=0, xmax=80,
ylabel={Latency [s]},
ymajorgrids,
ymin=0.75, ymax=0.9,
% ytick distance=1e-3,
]

\addplot [semithick, color0]
table {./figures/orderstats/data/azure/orderstats_2.csv};

\addplot [semithick, dashed, only marks, color2, mark=square*, mark size=1, mark options={fill=white,solid}] 
table {./figures/orderstats/data/azure/orderstats_gamma_gamma_2.csv};

\addplot [semithick, dashed, color3, mark=pentagon*, mark size=1, mark options={fill=white,solid}] 
table {./figures/orderstats/data/azure/orderstats_gamma_gamma_copula_2.csv};

\addplot [semithick, dashed, only marks, color1, mark=triangle*, mark size=1, mark options={fill=white,solid}] 
table {./figures/orderstats/data/azure/orderstats_global_gamma_2.csv};

\end{axis}%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% AWS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% aws bottom plot, job 3 (4.54e8)
\begin{axis}[
name=plot6,
at=(plot3.right of north east), anchor=left of north west,
legend cell align={left},
legend style={font=\scriptsize, fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.02,0.98)}, anchor=north west, draw=white!80!black},
tick pos=left,
tick label style={font=\scriptsize},
grid style={gray,opacity=0.5,dotted},
xlabel style={align=center}, xlabel={$w$},
xtick distance=20,
xmajorgrids,
height=\figureheight,
width=0.68\figurewidth,
xmin=0, xmax=80,
% ylabel={Latency [s]},
ymajorgrids,
ymin=0.58, ymax=0.66,
% ytick distance=1e-3,
]

\addplot [semithick, color0]
table {./figures/orderstats/data/aws/orderstats_3.csv};

\addplot [semithick, only marks, color2, mark=square*, mark size=1, mark options={fill=white,solid}] 
table {./figures/orderstats/data/aws/orderstats_gamma_gamma_3.csv};

\addplot [semithick, color3, only marks, mark=pentagon*, mark size=1, mark options={fill=white,solid}] 
table {./figures/orderstats/data/aws/orderstats_gamma_gamma_copula_3.csv};

\addplot [semithick, only marks, color1, mark=triangle*, mark size=1, mark options={fill=white,solid}] 
table {./figures/orderstats/data/aws/orderstats_global_gamma_3.csv};

\end{axis}
%
% aws middle plot, job 2 (1.13e7)
\begin{axis}[
name=plot5,
at=(plot6.above north east), anchor=below south east,
legend cell align={left},
legend style={font=\scriptsize, fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.02,0.98)}, anchor=north west, draw=white!80!black},
tick pos=left,
tick label style={font=\scriptsize},
grid style={gray,opacity=0.5,dotted},
xtick distance=20,
xmajorgrids,
height=\figureheight,
width=0.68\figurewidth,
xmin=0, xmax=80,
% ylabel={Latency [s]},
ymajorgrids,
ymin=1.2e-2, ymax=1.8e-2,
% ytick distance=1e-3,
]

\addplot [semithick, color0]
table {./figures/orderstats/data/aws/orderstats_2.csv};

\addplot [semithick, only marks, color2, mark=square*, mark size=1, mark options={fill=white,solid}] 
table {./figures/orderstats/data/aws/orderstats_gamma_gamma_2.csv};

\addplot [semithick, color3, only marks, mark=pentagon*, mark size=1, mark options={fill=white,solid}] 
table {./figures/orderstats/data/aws/orderstats_gamma_gamma_copula_2.csv};

\addplot [semithick, only marks, color1, mark=triangle*, mark size=1, mark options={fill=white,solid}] 
table {./figures/orderstats/data/aws/orderstats_global_gamma_2.csv};

\end{axis}%
%
% aws top plot, job 1 (2.84e6)
\begin{axis}[
name=plot4,
at=(plot5.above north east), anchor=below south east,
legend cell align={left},
legend style={font=\scriptsize, fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.02,0.98)}, anchor=north west, draw=white!80!black},
tick pos=left,
tick label style={font=\scriptsize},
grid style={gray,opacity=0.5,dotted},
xtick distance=20,
xmajorgrids,
height=\figureheight,
width=0.68\figurewidth,
xmin=0, xmax=80,
% ylabel={Latency [s]},
ymajorgrids,
ymin=3e-3, ymax=6e-3,
% ytick distance=1e-3,
]

\addplot [semithick, color0]
table {./figures/orderstats/data/aws/orderstats_1.csv};

\addplot [semithick, only marks, color2, mark=square*, mark size=1, mark options={fill=white,solid}] 
table {./figures/orderstats/data/aws/orderstats_gamma_gamma_1.csv};

\addplot [semithick, color3, only marks, mark=pentagon*, mark size=1, mark options={fill=white,solid}] 
table {./figures/orderstats/data/aws/orderstats_gamma_gamma_copula_1.csv};

\addplot [semithick, only marks, color1, mark=triangle*, mark size=1, mark options={fill=white,solid}] 
table {./figures/orderstats/data/aws/orderstats_global_gamma_1.csv};

\end{axis}%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% eX3 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% eX3 bottom plot, job 75 (4.67e8)
\begin{axis}[
name=plot9,
at=(plot6.right of north east), anchor=left of north west,
legend cell align={left},
legend style={font=\scriptsize, fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.02,0.98)}, anchor=north west, draw=white!80!black},
tick pos=left,
tick label style={font=\scriptsize},
grid style={gray,opacity=0.5,dotted},
xlabel style={align=center}, xlabel={$w$},
xtick distance=2,
xmajorgrids,
height=\figureheight,
width=0.68\figurewidth,
xmin=0, xmax=10,
% ylabel={Latency [s]},
ymajorgrids,
ymin=0.5, ymax=0.7,
% ytick distance=1e-3,
]

\addplot [semithick, color0]
table {./figures/orderstats/data/eX3/orderstats_75.csv};

\addplot [semithick, dashed, only marks, color2, mark=square*, mark size=1, mark options={fill=white,solid}] 
table {./figures/orderstats/data/eX3/orderstats_gamma_gamma_75.csv};

\addplot [semithick, dashed, color3, mark=pentagon*, mark size=1, mark options={fill=white,solid}] 
table {./figures/orderstats/data/eX3/orderstats_gamma_gamma_copula_75.csv};

\addplot [semithick, dashed, only marks, color1, mark=triangle*, mark size=1, mark options={fill=white,solid}] 
table {./figures/orderstats/data/eX3/orderstats_global_gamma_75.csv};

\end{axis}
%
% eX3 middle plot, job 3 (2.04e7)
\begin{axis}[
name=plot8,
at=(plot9.above north east), anchor=below south east,
legend cell align={left},
legend style={font=\scriptsize, fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.02,0.98)}, anchor=north west, draw=white!80!black},
tick pos=left,
tick label style={font=\scriptsize},
grid style={gray,opacity=0.5,dotted},
xtick distance=2,
xmajorgrids,
height=\figureheight,
width=0.68\figurewidth,
xmin=0, xmax=10,
% ylabel={Latency [s]},
ymajorgrids,
ymin=2.3e-2, ymax=2.7e-2,
% ytick distance=1e-3,
]

\addplot [semithick, color0]
table {./figures/orderstats/data/eX3/orderstats_3.csv};

\addplot [semithick, dashed, only marks, color2, mark=square*, mark size=1, mark options={fill=white,solid}] 
table {./figures/orderstats/data/eX3/orderstats_gamma_gamma_3.csv};

\addplot [semithick, dashed, color3, mark=pentagon*, mark size=1, mark options={fill=white,solid}] 
table {./figures/orderstats/data/eX3/orderstats_gamma_gamma_copula_3.csv};

\addplot [semithick, dashed, only marks, color1, mark=triangle*, mark size=1, mark options={fill=white,solid}] 
table {./figures/orderstats/data/eX3/orderstats_global_gamma_3.csv};

\end{axis}%
%
% eX3 top plot, job 66 (2.84e6)
\begin{axis}[
name=plot7,
at=(plot8.above north east), anchor=below south east,
legend cell align={left},
legend style={font=\scriptsize, fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.02,0.98)}, anchor=north west, draw=white!80!black},
tick pos=left,
tick label style={font=\scriptsize},
grid style={gray,opacity=0.5,dotted},
xtick distance=2,
xmajorgrids,
height=\figureheight,
width=0.68\figurewidth,
xmin=0, xmax=10,
% ylabel={Latency [s]},
ymajorgrids,
ymin=2.5e-3, ymax=4e-3,
% ytick distance=1e-3,
]

\addplot [semithick, color0]
table {./figures/orderstats/data/eX3/orderstats_66.csv};

\addplot [semithick, dashed, only marks, color2, mark=square*, mark size=1, mark options={fill=white,solid}] 
table {./figures/orderstats/data/eX3/orderstats_gamma_gamma_66.csv};

\addplot [semithick, dashed, color3, mark=pentagon*, mark size=1, mark options={fill=white,solid}] 
table {./figures/orderstats/data/eX3/orderstats_gamma_gamma_copula_66.csv};

\addplot [semithick, dashed, only marks, color1, mark=triangle*, mark size=1, mark options={fill=white,solid}] 
table {./figures/orderstats/data/eX3/orderstats_global_gamma_66.csv};

\end{axis}%
%
\end{tikzpicture}


==> figures/orderstats/orderstats1.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{HTML}{75b9be}
\definecolor{color1}{HTML}{ee7674}
\definecolor{color2}{HTML}{832161}
\definecolor{color3}{HTML}{eab464}
\definecolor{color4}{HTML}{335145}

\begin{axis}[
name=plot1,
legend cell align={left},
legend style={font=\scriptsize, fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.02,0.98)}, anchor=north west, draw=white!80!black},
% tick align=outside,
tick pos=left,
grid style={gray,opacity=0.5,dotted},
xlabel style={align=center}, xlabel={$w$},
xtick distance=10,
xmajorgrids,
height=\figureheight,
width=\figurewidth,
xmin=0, xmax=80,
ylabel={Latency [s]},
ymajorgrids,
% ymode=log,
ymin=4e-3, ymax=9e-3,
ytick distance=1e-3,
]

\addplot [semithick, color0]
table {./figures/orderstats/data/azure/orderstats_39.csv};
\addlegendentry{Empirical}

\addplot [semithick, dashed, only marks, color2, mark=square*, mark size=1, mark options={fill=white,solid}] 
% table {./figures/orderstats/data/azure/orderstats_shiftexp_shiftexp_39.csv};
table {./figures/orderstats/data/azure/orderstats_gamma_gamma_39.csv};
\addlegendentry{Predicted}
% \addlegendentry{Shift. exp. (ind.)}

\addplot [semithick, dashed, only marks, color1, mark=triangle*, mark size=1, mark options={fill=white,solid}] 
% table {./figures/orderstats/data/azure/orderstats_global_shiftexp_39.csv};
table {./figures/orderstats/data/azure/orderstats_global_gamma_39.csv};
\addlegendentry{Predicted (i.i.d.)}
% \addlegendentry{Shift. exp. (i.i.d.)}

% \addplot [semithick, dashed, color3, mark=pentagon*, mark size=1, mark options={fill=white,solid}] 
% table {./figures/orderstats/data/azure/orderstats_shiftexp_shiftexp_copula_10.csv};
% \addlegendentry{Model}
% \addlegendentry{Shift. exp.}

% \addplot [semithick, dashed, color2, mark=triangle*, mark size=1, mark options={fill=white,solid}] 
% table {./figures/orderstats/data/azure/orderstats_global_gamma_10.csv};
% \addlegendentry{Gamma (i.i.d.)}

% \addplot [semithick, dashed, color2, mark=square*, mark size=1, mark options={fill=white,solid}] 
% table {./figures/orderstats/data/azure/orderstats_gamma_gamma_10.csv};
% \addlegendentry{Gamma (ind.)}

% \addplot [semithick, dashed, color2, mark=pentagon*, mark size=1, mark options={fill=white,solid}] 
% table {./figures/orderstats/data/azure/orderstats_gamma_gamma_copula_10.csv};
% \addlegendentry{Gamma}

\end{axis}

\end{tikzpicture}


==> figures/timeseries/grid.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{HTML}{75b9be}
\definecolor{color1}{HTML}{ee7674}
\definecolor{color2}{HTML}{832161}
\definecolor{color3}{HTML}{eab464}
\definecolor{color4}{HTML}{335145}

% adjust line length in legend to show which line is dashed
\pgfplotsset{
legend image code/.code={
\draw[mark repeat=2,mark phase=2]
plot coordinates {
(0cm,0cm)
(0.2cm,0cm)        %% default is (0.3cm,0cm)
(0.4cm,0cm)         %% default is (0.6cm,0cm)
};%
}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  Azure %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
% Azure job 39 iteration 1001-1600 (2.84e6)
\begin{axis}[
name=plot1,
axis y line*=left,
legend cell align={left},
legend style={font=\scriptsize, fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.02,0.98)}, anchor=north west, draw=white!80!black},
tick pos=left,
tick label style={font=\scriptsize},
% scaled y ticks=false,
grid style={gray,opacity=0.5,dotted},
% xlabel style={align=center}, xlabel={Iteration},
xtick distance=20,
xmajorgrids,
height=\figureheight,
width=0.65\figurewidth,
xmin=0, xmax=100,
ylabel={Latency (comp.) [s]},
ymajorgrids,
ymin=0e-3, ymax=6e-3,
% ytick distance=1e-3,
]

% comp.
\addplot [semithick, color0, mark=triangle*, mark size=1, mark options={fill=white}] 
table {./figures/timeseries/data/Azure/timeseries_compute_39_1.csv};
\addlegendentry{Worker $1$ (comp.)}
\addplot [semithick, color1, densely dashed, mark=triangle*, mark size=1, mark options={fill=white, solid}] 
table {./figures/timeseries/data/Azure/timeseries_compute_39_11.csv};
\addlegendentry{Worker $2$ (comp.)}

\addplot [semithick, color0, mark=*, mark size=1, mark options={fill=white}] 
table {
-1 0
};
\addlegendentry{Worker $1$ (comm.)}

\addplot [semithick, color1, densely dashed, mark=*, mark size=1, mark options={fill=white, solid}]
table {
-1 0
};
\addlegendentry{Worker $2$ (comm.)}

\end{axis}%
%
% comm.
\begin{axis}[
name=plot1comm,
at=(plot1.north west), anchor=north west,
axis y line*=right,
axis x line=none,
tick pos=right,
tick label style={font=\scriptsize},
% scaled y ticks=false,
height=\figureheight,
width=0.65\figurewidth,
xmin=0, xmax=100,
ymin=0e-3, ymax=6e-3,
% ylabel={Latency (comm.) [s]},
% ytick distance=1e-3,
]
\addplot [semithick, color0, mark=*, mark size=1, mark options={fill=white}] 
table {./figures/timeseries/data/Azure/timeseries_communication_39_1.csv};
\addplot [semithick, color1, densely dashed, mark=*, mark size=1, mark options={fill=white, solid}] 
table {./figures/timeseries/data/Azure/timeseries_communication_39_11.csv};

\end{axis}%
%
% Azure job 35 iteration 1-100   (1.13e7)
\begin{axis}[
name=plot2,
at=(plot1.below south west), anchor=above north west,
legend cell align={left},
legend style={font=\scriptsize, fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.02,0.98)}, anchor=north west, draw=white!80!black},
tick pos=left,
tick label style={font=\scriptsize},
grid style={gray,opacity=0.5,dotted},
% xlabel style={align=center}, xlabel={Iteration},
xtick distance=20,
xmajorgrids,
height=\figureheight,
width=0.65\figurewidth,
xmin=0, xmax=100,
ylabel={Latency (comp.) [s]},
ymajorgrids,
ymin=1e-2, ymax=2e-2,
% ytick distance=1e-3,
]

% comp.
\addplot [semithick, color0, mark=triangle*, mark size=1, mark options={fill=white}] 
table {./figures/timeseries/data/Azure/timeseries_compute_35_1.csv};
\addplot [semithick, color1, densely dashed, mark=triangle*, mark size=1, mark options={fill=white, solid}]  
table {./figures/timeseries/data/Azure/timeseries_compute_35_2.csv};

\end{axis}%
%
% comm.
\begin{axis}[
name=plot2comm,
at=(plot2.north west), anchor=north west,
axis y line*=right,
axis x line=none,
tick pos=right,
tick label style={font=\scriptsize},
height=\figureheight,
width=0.65\figurewidth,
xmin=0, xmax=100,
ymin=0e-3, ymax=6e-3,
% ylabel={Latency (comm.) [s]},
% ytick distance=1e-3,
]
\addplot [semithick, color0, mark=*, mark size=1, mark options={fill=white}] 
table {./figures/timeseries/data/Azure/timeseries_communication_35_1.csv};
\addplot [semithick, color1, densely dashed, mark=*, mark size=1, mark options={fill=white, solid}] 
table {./figures/timeseries/data/Azure/timeseries_communication_35_2.csv};

\end{axis}%
%
% Azure job 2 (4.54e8)
% comm.
\begin{axis}[
name=plot3,
at=(plot2.below south west), anchor=above north west,
axis y line*=right,
axis x line=none,
tick pos=right,
tick label style={font=\scriptsize},
height=\figureheight,
width=0.65\figurewidth,
xmin=0, xmax=100,
ymin=0e-3, ymax=6e-3,
% ylabel={Latency (comm.) [s]},
% ytick distance=1e-3,
]
\addplot [semithick, color0, mark=*, mark size=1, mark options={fill=white}] 
table {./figures/timeseries/data/Azure/timeseries_communication_2_3.csv};
\addplot [semithick, color1, densely dashed, mark=*, mark size=1, mark options={fill=white, solid}] 
table {./figures/timeseries/data/Azure/timeseries_communication_2_4.csv};

\end{axis}%
% comp
\begin{axis}[
name=plot3comp,
at=(plot3.north west), anchor=north west,
legend cell align={left},
legend style={font=\scriptsize, fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.02,0.98)}, anchor=north west, draw=white!80!black},
tick pos=left,
tick label style={font=\scriptsize},
grid style={gray,opacity=0.5,dotted},
xlabel style={align=center}, xlabel={Iteration},
xtick distance=20,
xmajorgrids,
height=\figureheight,
width=0.65\figurewidth,
xmin=0, xmax=80,
ylabel={Latency (comp.) [s]},
ymajorgrids,
ymin=0.7, ymax=0.8,
% ytick distance=1e-3,
]

% comp.
\addplot [semithick, color0, mark=triangle*, mark size=1, mark options={fill=white}] 
table {./figures/timeseries/data/Azure/timeseries_compute_2_3.csv};
\addplot [semithick, color1, densely dashed, mark=triangle*, mark size=1, mark options={fill=white, solid}] 
table {./figures/timeseries/data/Azure/timeseries_compute_2_4.csv};

\end{axis}%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% AWS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
% AWS bottom plot, job 3 iteration 1-100 (4.54e8)
\begin{axis}[
name=plot6,
at=(plot3.right of north east), anchor=left of north west,
legend cell align={left},
legend style={font=\scriptsize, fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.02,0.98)}, anchor=north west, draw=white!80!black},
tick pos=left,
tick label style={font=\scriptsize},
grid style={gray,opacity=0.5,dotted},
xlabel style={align=center}, xlabel={Iteration},
xtick distance=20,
xmajorgrids,
height=\figureheight,
width=0.65\figurewidth,
xmin=0, xmax=100,
% ylabel={Latency [s]},
ymajorgrids,
ymin=0.6, ymax=0.64,
% ytick distance=1e-3,
]

% comp.
\addplot [semithick, color0, mark=triangle*, mark size=1, mark options={fill=white}] 
table {./figures/timeseries/data/aws/timeseries_compute_3_1.csv};
\addplot [semithick, color1, densely dashed, mark=triangle*, mark size=1, mark options={fill=white, solid}] 
table {./figures/timeseries/data/aws/timeseries_compute_3_2.csv};
\end{axis}%
%
% comm.
\begin{axis}[
name=plot6comm,
at=(plot6.north west), anchor=north west,
axis y line*=right,
axis x line=none,
tick pos=right,
tick label style={font=\scriptsize},
height=\figureheight,
width=0.65\figurewidth,
xmin=0, xmax=100,
ymin=0e-3, ymax=6e-3,
% ylabel={Latency (comm.) [s]},
% ytick distance=1e-3,
]
\addplot [semithick, color0, mark=*, mark size=1, mark options={fill=white}] 
table {./figures/timeseries/data/aws/timeseries_communication_3_1.csv};
\addplot [semithick, color1, densely dashed, mark=*, mark size=1, mark options={fill=white, solid}] 
table {./figures/timeseries/data/aws/timeseries_communication_3_2.csv};
\end{axis}%
%
% AWS middle plot, job 2 iteration 1-100 (1.13e7)
\begin{axis}[
name=plot5,
at=(plot6comm.above north east), anchor=below south east,
legend cell align={left},
legend style={font=\scriptsize, fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.02,0.98)}, anchor=north west, draw=white!80!black},
tick pos=left,
tick label style={font=\scriptsize},
grid style={gray,opacity=0.5,dotted},
% xlabel style={align=center}, xlabel={Iteration},
xtick distance=20,
xmajorgrids,
height=\figureheight,
width=0.65\figurewidth,
xmin=0, xmax=100,
% ylabel={Latency [s]},
ymajorgrids,
ymin=1e-2, ymax=2e-2,
% ytick distance=1e-3,
]

% comp.
\addplot [semithick, color0, mark=triangle*, mark size=1, mark options={fill=white}] 
table {./figures/timeseries/data/aws/timeseries_compute_2_1.csv};
\addplot [semithick, color1, densely dashed, mark=triangle*, mark size=1, mark options={fill=white, solid}] 
table {./figures/timeseries/data/aws/timeseries_compute_2_2.csv};
\end{axis}%
%
% comm.
\begin{axis}[
name=plot5comm,
at=(plot5.north west), anchor=north west,
axis y line*=right,
axis x line=none,
tick pos=right,
tick label style={font=\scriptsize},
height=\figureheight,
width=0.65\figurewidth,
xmin=0, xmax=100,
ymin=0e-3, ymax=6e-3,
% ylabel={Latency (comm.) [s]},
% ytick distance=1e-3,
]
\addplot [semithick, color0, mark=*, mark size=1, mark options={fill=white}] 
table {./figures/timeseries/data/aws/timeseries_communication_2_1.csv};
\addplot [semithick, color1, densely dashed, mark=*, mark size=1, mark options={fill=white, solid}] 
table {./figures/timeseries/data/aws/timeseries_communication_2_2.csv};
\end{axis}%
%
% AWS top plot, job 1 iteration 1-100 (2.84e6)
\begin{axis}[
name=plot4,
at=(plot5comm.above north east), anchor=below south east,
legend cell align={left},
legend style={font=\scriptsize, fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.02,0.98)}, anchor=north west, draw=white!80!black},
tick pos=left,
tick label style={font=\scriptsize},
grid style={gray,opacity=0.5,dotted},
% xlabel style={align=center}, xlabel={Iteration},
xtick distance=20,
xmajorgrids,
height=\figureheight,
width=0.65\figurewidth,
xmin=0, xmax=100,
% ylabel={Latency [s]},
ymajorgrids,
ymin=0e-3, ymax=6e-3,
% ytick distance=1e-3,
]

% comp.
\addplot [semithick, color0, mark=triangle*, mark size=1, mark options={fill=white}] 
table {./figures/timeseries/data/aws/timeseries_compute_1_1.csv};
\addplot [semithick, color1, densely dashed, mark=triangle*, mark size=1, mark options={fill=white, solid}] 
table {./figures/timeseries/data/aws/timeseries_compute_1_2.csv};
\end{axis}%
%
% comm.
\begin{axis}[
name=plot4comm,
at=(plot4.north west), anchor=north west,
axis y line*=right,
axis x line=none,
tick pos=right,
tick label style={font=\scriptsize},
height=\figureheight,
width=0.65\figurewidth,
xmin=0, xmax=100,
ymin=0e-3, ymax=6e-3,
% ylabel={Latency (comm.) [s]},
% ytick distance=1e-3,
]
\addplot [semithick, color0, mark=*, mark size=1, mark options={fill=white}] 
table {./figures/timeseries/data/aws/timeseries_communication_1_1.csv};
\addplot [semithick, color1, densely dashed, mark=*, mark size=1, mark options={fill=white, solid}] 
table {./figures/timeseries/data/aws/timeseries_communication_1_2.csv};
\end{axis}%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% eX3 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
% eX3 bottom plot, job 75 (4.67e8)
\begin{axis}[
name=plot9,
at=(plot6.right of north east), anchor=left of north west,
legend cell align={left},
legend style={font=\scriptsize, fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.02,0.98)}, anchor=north west, draw=white!80!black},
tick pos=left,
tick label style={font=\scriptsize},
grid style={gray,opacity=0.5,dotted},
xlabel style={align=center}, xlabel={Iteration},
xtick distance=20,
xmajorgrids,
height=\figureheight,
width=0.65\figurewidth,
xmin=0, xmax=100,
% ylabel={Latency [s]},
ymajorgrids,
ymin=0.55, ymax=0.75,
% ytick distance=1e-3,
]

% comp.
\addplot [semithick, color0, mark=triangle*, mark size=1, mark options={fill=white}] 
table {./figures/timeseries/data/eX3/timeseries_compute_75_1.csv};
\addplot [semithick, color1, densely dashed, mark=triangle*, mark size=1, mark options={fill=white, solid}]
table {./figures/timeseries/data/eX3/timeseries_compute_75_2.csv};

\end{axis}%
%
% comm.
\begin{axis}[
name=plot9comm,
at=(plot9.north west), anchor=north west,
axis y line*=right,
axis x line=none,
tick pos=right,
tick label style={font=\scriptsize},
height=\figureheight,
width=0.65\figurewidth,
xmin=0, xmax=100,
ylabel={Latency (comm.) [s]},
ymin=0e-5, ymax=6e-5,
% ytick distance=1e-3,
]
\addplot [semithick, color0, mark=*, mark size=1, mark options={fill=white}] 
table {./figures/timeseries/data/eX3/timeseries_communication_75_1.csv};
\addplot [semithick, color1, densely dashed, mark=*, mark size=1, mark options={fill=white, solid}]
table {./figures/timeseries/data/eX3/timeseries_communication_75_2.csv};
\end{axis}%
%
% eX3 middle plot, job 3 iteration 451-550 (2.04e7)
\begin{axis}[
name=plot8,
at=(plot9comm.above north east), anchor=below south east,
legend cell align={left},
legend style={font=\scriptsize, fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.02,0.98)}, anchor=north west, draw=white!80!black},
tick pos=left,
tick label style={font=\scriptsize},
grid style={gray,opacity=0.5,dotted},
% xlabel style={align=center}, xlabel={Iteration},
xtick distance=20,
xmajorgrids,
height=\figureheight,
width=0.65\figurewidth,
xmin=0, xmax=100,
% ylabel={Latency [s]},
ymajorgrids,
ymin=1e-2, ymax=3e-2,
% ytick distance=1e-3,
]

% comp.
\addplot [semithick, color0, mark=triangle*, mark size=1, mark options={fill=white}] 
table {./figures/timeseries/data/eX3/timeseries_compute_3_1.csv};
\addplot [semithick, color1, densely dashed, mark=triangle*, mark size=1, mark options={fill=white, solid}] 
table {./figures/timeseries/data/eX3/timeseries_compute_3_2.csv};

\end{axis}%
%
% comm.
\begin{axis}[
name=plot8comm,
at=(plot8.north west), anchor=north west,
axis y line*=right,
axis x line=none,
tick pos=right,
tick label style={font=\scriptsize},
height=\figureheight,
width=0.65\figurewidth,
xmin=0, xmax=100,
ylabel={Latency (comm.) [s]},
ymin=0e-5, ymax=6e-5,
% ytick distance=1e-3,
]
\addplot [semithick, color0, mark=*, mark size=1, mark options={fill=white}] 
table {./figures/timeseries/data/eX3/timeseries_communication_3_1.csv};
\addplot [semithick, color1, densely dashed, mark=*, mark size=1, mark options={fill=white, solid}]
table {./figures/timeseries/data/eX3/timeseries_communication_3_2.csv};
\end{axis}%
%
% eX3 top plot, job 66  iteration 751-850 (2.84e6)
\begin{axis}[
name=plot7,
at=(plot8comm.above north east), anchor=below south east,
legend cell align={left},
legend style={font=\scriptsize, fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.02,0.98)}, anchor=north west, draw=white!80!black},
tick pos=left,
tick label style={font=\scriptsize},
grid style={gray,opacity=0.5,dotted},
% xlabel style={align=center}, xlabel={Iteration},
xtick distance=20,
xmajorgrids,
height=\figureheight,
width=0.65\figurewidth,
xmin=0, xmax=100,
% ylabel={Latency [s]},
ymajorgrids,
ymin=0e-3, ymax=6e-3,
% ytick distance=1e-3,
]

% comp.
\addplot [semithick, color0, mark=triangle*, mark size=1, mark options={fill=white}] 
table {./figures/timeseries/data/eX3/timeseries_compute_66_1.csv};
\addplot [semithick, color1, densely dashed, mark=triangle*, mark size=1, mark options={fill=white, solid}] 
table {./figures/timeseries/data/eX3/timeseries_compute_66_2.csv};

\end{axis}%
%
% comm.
\begin{axis}[
name=plot7comm,
at=(plot7.north west), anchor=north west,
axis y line*=right,
axis x line=none,
tick pos=right,
tick label style={font=\scriptsize},
height=\figureheight,
width=0.65\figurewidth,
xmin=0, xmax=100,
ylabel={Latency (comm.) [s]},
ymin=0e-5, ymax=6e-5,
% ytick distance=1e-3,
]
\addplot [semithick, color0, mark=*, mark size=1, mark options={fill=white}] 
table {./figures/timeseries/data/eX3/timeseries_communication_66_1.csv};
\addplot [semithick, color1, densely dashed, mark=*, mark size=1, mark options={fill=white, solid}]
table {./figures/timeseries/data/eX3/timeseries_communication_66_2.csv};
\end{axis}%
%
\end{tikzpicture}


==> figures/timeseries/grid_comm.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{HTML}{75b9be}
\definecolor{color1}{HTML}{ee7674}
\definecolor{color2}{HTML}{832161}
\definecolor{color3}{HTML}{eab464}
\definecolor{color4}{HTML}{335145}

% adjust line length in legend to show which line is dashed
\pgfplotsset{
legend image code/.code={
\draw[mark repeat=2,mark phase=2]
plot coordinates {
(0cm,0cm)
(0.2cm,0cm)        %% default is (0.3cm,0cm)
(0.4cm,0cm)         %% default is (0.6cm,0cm)
};%
}
}

% Azure job 39 iteration 1001-1600 (2.84e6)
\begin{axis}[
name=plot1,
legend cell align={left},
legend style={font=\scriptsize, fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.02,0.98)}, anchor=north west, draw=white!80!black},
tick pos=left,
grid style={gray,opacity=0.5,dotted},
xlabel style={align=center}, xlabel={Iteration},
xtick distance=10,
xmajorgrids,
height=\figureheight,
width=\figurewidth,
xmin=0, xmax=100,
ylabel={Latency [s]},
ymajorgrids,
% ymin=4e-3, ymax=9e-3,
% ytick distance=1e-3,
]

% comm.
\addplot [semithick, color0, mark=square*, mark size=2, mark options={fill=white}] table {./figures/timeseries/data/Azure/timeseries_communication_39_1.csv};
\addlegendentry{Worker $1$}
\addplot [semithick, color1, densely dashed, mark=*, mark size=2, mark options={fill=white, solid}] table {./figures/timeseries/data/Azure/timeseries_communication_39_11.csv};
\addlegendentry{Worker $2$}

\end{axis}%
%
% eX3 job 66  iteration 751-850 (2.84e6)
\begin{axis}[
name=plot7,
at=(plot1.north east), anchor=left of north west,
legend cell align={left},
legend style={font=\scriptsize, fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.02,0.98)}, anchor=north west, draw=white!80!black},
tick pos=left,
grid style={gray,opacity=0.5,dotted},
xlabel style={align=center}, xlabel={Iteration},
xtick distance=10,
xmajorgrids,
height=\figureheight,
width=\figurewidth,
xmin=0, xmax=100,
ylabel={Latency [s]},
ymajorgrids,
% ymin=4e-3, ymax=9e-3,
% ytick distance=1e-3,
]

% comm.
\addplot [semithick, color0, mark=square*, mark size=2, mark options={fill=white}] 
table {./figures/timeseries/data/eX3/timeseries_communication_66_1.csv};
\addplot [semithick, color1, densely dashed, mark=*, mark size=2, mark options={fill=white, solid}]
table {./figures/timeseries/data/eX3/timeseries_communication_66_2.csv};

\end{axis}

\end{tikzpicture}

